Worst-Case Detection Performance for Distributed SIMO Physical Layer Authentication

Feature-based physical layer authentication (PLA) schemes, using position-specific channel characteristics as identifying features, can provide lightweight protection against impersonation attacks in overhead-limited applications like e.g., mission-critical and low-latency scenarios. However, with PLA-aware attack strategies, an attacker can maximize the probability of successfully impersonating the legitimate devices. In this paper, we provide worst-case detection performance bounds under such strategies for a distributed PLA scheme that is based on the channel-state information (CSI) observed at multiple distributed remote radio-heads. This distributed setup exploits the multiple-channel diversity for enhanced detection performance and mimics distributed antenna architectures considered for 4G and 5G radio access networks. We consider (i) a power manipulation attack, in which a single-antenna attacker adopts optimal transmit power and phase; and (ii) an optimal spatial position attack. Interestingly, our results show that the attacker can achieve close-to-optimal success probability with only statistical CSI, which significantly strengthens the relevance of our results for practical scenarios. Furthermore, our results show that, by distributing antennas to multiple radio-heads, the worst-case missed detection probability can be reduced by 4 orders of magnitude without increasing the total number of antennas, illustrating the superiority of distributed PLA over a co-located antenna setup.

==> config/packages.tex <==
%\usepackage{nopageno}
\usepackage{psfrag}
\usepackage[final,dvips]{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{epsfig}
\usepackage{amsthm}
\usepackage[square,numbers,sort&compress]{natbib}
\usepackage[table,xcdraw]{xcolor}
\usepackage{array}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{mathtools}
\usepackage[english]{babel}
\usepackage{tikz}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother

\usepackage[labelformat=simple]{subcaption}
\renewcommand\thesubfigure{(\alph{subfigure})}
\usepackage{booktabs}
\DeclareCaptionLabelSeparator{periodspace}{.\quad}
\captionsetup{font=footnotesize,labelsep=periodspace,singlelinecheck=false}
\captionsetup[sub]{font=footnotesize,singlelinecheck=true}
\newcommand\equationspace{\vspace{-1.5ex}}

\captionsetup[figure]{name={Fig.},labelsep=period}

\DeclareGraphicsExtensions{.pdf,.png,.jpg,.eps}
\DeclareGraphicsRule{pst}{eps}{pst}{}

\bibliographystyle{IEEEtran}




==> parts/app_scenarios.tex <==




\begin{figure*}[h!]
\caption{\textbf{Scenario A}: (a) map (b) performance.}
\begin{subfigure}{0.5\textwidth}
\psfrag{X}[][]{\small $x$ [m]}
\psfrag{Y}[][]{\small $y$ [m]}
\includegraphics[width=\columnwidth]{figures/Scenarios/scenA_map.eps}
\caption{}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
\psfrag{X}[][]{\tiny Position index}
\psfrag{YA}[][]{\tiny \textcolor{matlab-blue}{Objective function $f_{\text{obj}}(\mean_E)$}}
\psfrag{YB}[][][1][-180]{\tiny \textcolor{matlab-red}{Missed detection prob. $\pMD^{(wc)}$}}
\includegraphics[width=\columnwidth]{figures/Scenarios/scenA_performance.eps}
\caption{}
\end{subfigure} %
\end{figure*}



\begin{figure*}[h!]
\centering
\caption{\textbf{Scenario B}: (a) map (b) performance.}
\begin{subfigure}{0.5\textwidth}
\psfrag{X}[][]{\small $x$ [m]}
\psfrag{Y}[][]{\small $y$ [m]}
\includegraphics[width=\columnwidth]{figures/Scenarios/scenB_map.eps}
\caption{}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
\psfrag{X}[][]{\tiny Position index}
\psfrag{YA}[][]{\tiny \textcolor{matlab-blue}{Objective function $f_{\text{obj}}(\mean_E)$}}
\psfrag{YB}[][][1][-180]{\tiny \textcolor{matlab-red}{Missed detection prob. $\pMD^{(wc)}$}}
\includegraphics[width=\columnwidth]{figures/Scenarios/scenB_performance.eps}
\caption{}
\end{subfigure} %
\end{figure*}


\begin{figure*}[h!]
\centering
\caption{\textbf{Scenario C}: (a) map (b) performance.}
\begin{subfigure}{0.5\textwidth}
\psfrag{X}[][]{\small $x$ [m]}
\psfrag{Y}[][]{\small $y$ [m]}
\includegraphics[width=\columnwidth]{figures/Scenarios/scenC_map.eps}
\caption{}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
\psfrag{X}[][]{\tiny Position index}
\psfrag{YA}[][]{\tiny \textcolor{matlab-blue}{Objective function $f_{\text{obj}}(\mean_E)$}}
\psfrag{YB}[][][1][-180]{\tiny \textcolor{matlab-red}{Missed detection prob. $\pMD^{(wc)}$}}
\includegraphics[width=\columnwidth]{figures/Scenarios/scenC_performance.eps}
\caption{}
\end{subfigure} %
\end{figure*}


\begin{figure*}[h!]
\centering
\caption{\textbf{Scenario D}: (a) map (b) performance.}
\begin{subfigure}{0.5\textwidth}
\psfrag{X}[][]{\small $x$ [m]}
\psfrag{Y}[][]{\small $y$ [m]}
\includegraphics[width=\columnwidth]{figures/Scenarios/scenD_map.eps}
\caption{}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
\psfrag{X}[][]{\tiny Position index}
\psfrag{YA}[][]{\tiny \textcolor{matlab-blue}{Objective function $f_{\text{obj}}(\mean_E)$}}
\psfrag{YB}[][][1][-180]{\tiny \textcolor{matlab-red}{Missed detection prob. $\pMD^{(wc)}$}}
\includegraphics[width=\columnwidth]{figures/Scenarios/scenD_performance.eps}
\caption{}
\end{subfigure} %
\end{figure*}


\begin{figure*}[h!]
\centering
\caption{\textbf{Scenario E}: (a) map (b) performance.}
\begin{subfigure}{0.5\textwidth}
\psfrag{X}[][]{\small $x$ [m]}
\psfrag{Y}[][]{\small $y$ [m]}
\includegraphics[width=\columnwidth]{figures/Scenarios/scenE_map.eps}
\caption{}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
\psfrag{X}[][]{\tiny Position index}
\psfrag{YA}[][]{\tiny \textcolor{matlab-blue}{Objective function $f_{\text{obj}}(\mean_E)$}}
\psfrag{YB}[][][1][-180]{\tiny \textcolor{matlab-red}{Missed detection prob. $\pMD^{(wc)}$}}
\includegraphics[width=\columnwidth]{figures/Scenarios/scenE_performance.eps}
\caption{}
\end{subfigure} %
\end{figure*}


\begin{figure*}[h!]
\centering
\caption{\textbf{Scenario F}: (a) map (b) performance.}
\begin{subfigure}{0.5\textwidth}
\psfrag{X}[][]{\small $x$ [m]}
\psfrag{Y}[][]{\small $y$ [m]}
\includegraphics[width=\columnwidth]{figures/Scenarios/scenF_map.eps}
\caption{}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
\psfrag{X}[][]{\tiny Position index}
\psfrag{YA}[][]{\tiny \textcolor{matlab-blue}{Objective function $f_{\text{obj}}(\mean_E)$}}
\psfrag{YB}[][][1][-180]{\tiny \textcolor{matlab-red}{Missed detection prob. $\pMD^{(wc)}$}}
\includegraphics[width=\columnwidth]{figures/Scenarios/scenF_performance.eps}
\caption{}
\end{subfigure} %
\end{figure*}

\begin{figure*}[h!]
\centering
\caption{\textbf{Scenario G}: (a) map (b) performance.}
\begin{subfigure}{0.5\textwidth}
\psfrag{X}[][]{\small $x$ [m]}
\psfrag{Y}[][]{\small $y$ [m]}
\includegraphics[width=\columnwidth]{figures/Scenarios/scenG_map.eps}
\caption{}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
\psfrag{X}[][]{\tiny Position index}
\psfrag{YA}[][]{\tiny \textcolor{matlab-blue}{Objective function $f_{\text{obj}}(\mean_E)$}}
\psfrag{YB}[][][1][-180]{\tiny \textcolor{matlab-red}{Missed detection prob. $\pMD^{(wc)}$}}
\includegraphics[width=\columnwidth]{figures/Scenarios/scenG_performance.eps}
\caption{}
\end{subfigure} %
\end{figure*}

==> parts/proof_chernoff.tex <==
We start by upper bounding \eqref{eq:p_MD_L2} according to

\begin{equation}
	\label{eq:chernoff1}
\begin{aligned}
\pMD^{L=2}(T) &\leq \prob(d(\h_E)<d(\h_A)) \\
&= \prob(e^{t(d(\h_A)-d(\h_E))}>1) \\
&\leq \E[e^{-td(\h_E)}]\E[e^{td(\h_A)}],
\end{aligned}
\end{equation}
%
which holds for any $t>0$ due to the Markov inequality and the fact that $\h_E$ is assumed independent of $\h_A$.
We have previously concluded that $d(\h_A)\sim \chi^2_{2\Ka\NRx}$ from which it follows that the moment generating function (MGF) $\E[e^{td(\h_A)}] = (1-2t)^{-\Ka\NRx}$.
Due to the independent fading of the channels from Eve to each receive array, we can decompose 
$d(\h_E)=\sum_{k=1}^{\Ka} d^{(k)}(\h_E^{(k)})$ (see Remark~\ref{re:local_discriminant}).
Now, using the assumption that 
$\Cov_E^{(k)} = \frac{P_E^{(k)}}{\KRice+1}\A$ 
and 
$\Cov_A^{(k)} = \frac{P_A^{(k)}}{\KRice+1}\A$, 
we get that 
$\Cov_E^{(k)} = \alpha_k\Cov_A^{(k)}$ with 
$\alpha_k = \frac{P_E^{(k)}}{P_A^{(k)}}$, and hence, $d^{(k)}(\h_E^{(k)})=\alpha_kY_k$ with

\begin{equation}
	Y_k = 2\QF[{ [\Cov_{E}^{(k)}]^{-1}}]{\h_E^{(k)}-\mean_{A}^{(k)}}
\end{equation}
%
It is known that $Y_k\sim\chi_{2\NRx}^{2}(\nu_k)$, independent over $k$, with non-centrality parameters 
$\nu_k = \QF[{[\Cov_{E}^{(k)}]^{-1}}]{\mean_{E}^{(k)}-\mean_{A}^{(k)} }$.
The MGF can be factorized as 
$\E[e^{-td(\h_E)}]=\E[e^{-t\sum_{k=1}^{\Ka}\alpha_kY_k}]=\prod_{k=1}^{\Ka}\E[e^{-t\alpha_k Y_k}]$.
Finally, the factors
$\E[e^{-t\alpha_k Y_k}] = (1+2\alpha_k t)^{-\NRx}\exp\left(\frac{-\nu_k \alpha_k t}{1+2 \alpha_k t}\right)$
which is the standard MGF of a non-central $\chi^2$ distribution.
Plugging this into \eqref{eq:chernoff1} and minimizing over $t$ yields \eqref{eq:chernoff}.

%$2(\h_E^{(k)}-\mean_{A}^{(k)} )^\dag [\Cov_{i}^{(A)}]^{-1}(\h_E^{(k)}-\mean_{A}^{(k)})$


 % and $d_i(\h_E)\sim \lambda\chi^2_{2\NRx}(\nu_i)$ (see Section~\ref{subsec:far_mdr}), we get $\E[e^{td_i(\h_i)}] = (1-2t)^{-\NRx}$ and $\E[e^{-td_i(\h_E)}] = (1+2\lambda t)^{-\NRx}\exp\left(\frac{-\nu_i \lambda t}{1+2 \lambda t}\right)$ for $-\lambda/2<t<1/2$ from the standard moment generating functions for the corresponding distributions.
 %


% and it is clear that
% $d(\tilde{\h}) = \sum_{k=1}^{\Ka}\alpha_k Y_k$ with $Y_k = 2(\tilde{\h}_k-\mean_{A,k})^\dag\Cov_{A,k}^{-1}(\tilde{\h}_k-\mean_{A,k})$. It is straightforward to prove that $Y_k $ is distributed according to $\chi_{2\NRx}^2(\nu_i)$~\cite{Forssell2018Arxiv}.

==> parts/queueing_analysis.tex <==
In this section, we integrate the distributed system model into previously developed tools for analyzing the delay performance impacts of PLA.
We begin by reviewing some preliminary concepts related to stochastic network calculus and a bound on the delay violation probability.
For a complete and detailed understanding of these concepts in relation to PLA, we refer the reader to~\cite{Forssell2019}.
The main contribution of this section is the derivation of the service process for the distributed setting under both local and centralized processing and with cenral PLA decisions.

\subsection{Preliminaries} % (fold)
\label{sub:preliminaries}

The use of PLA for enhanced security might have unintended consequences on the system's ability to meet delay requirements. 
To study such delay performance issues, we introduce infinite-buffer queues that model the flow of data from each device to the CPU.
We let the discrete-time queueing system be modeled by the bivariate stochastic processes $A_i(\tau,t) = \sum_{k=\tau}^{t}a_{k,i}$ and $D_i(\tau,t) = \sum_{k=\tau}^{t}d_{k,i}$, that denote the cumulative arrivals to and departures from link $i$, respectively, for all $0 \le \tau \le t$.
Here $a_{k,i}$ represents the instantaneous arrivals to the device's buffer in frame $k$ measured in bits.
Similarly, $d_{k,i}$ represents the instantaneous departures from the queue (i.e., information successfully received, decoded, and authenticated at the CPU).
The link's ability to transfer data from the local buffer to the CPU is characterized by the cumulative service process $S_i(\tau,t) = \sum_{k=\tau}^{t}s_{k,i}$, where $s_{k,i}$ represents the instantaneous service in frame $k$; that is, $s_{k,i}$ is the amount of information bits that can be reliably communicated over the wireless channels to the distributed arrays and sucessfully received, decoded, and authenticated at the CPU.

\paragraph{Delay Violation Probability}
\label{par:delay_violation_probability}

The queueing delay at time point $t$ is defined as

\begin{equation}
W_i(t) \triangleq \inf \{u>0;A_i(0,t)\leq D_i(0,t+u)\},
\end{equation}
%
representing the frames required to serve the bits in the queue at time $t$. 
This delay is randomly varying due to the stochastic service process.
A widely used measure on the queueing system's ability to meet delay requirements is the \textit{delay violation probability}~\cite{Zubaidy2016}, defined as $p_i(w) = \mathbb{P}(W_i(t)>w)$, i.e., the probability that a bit is not received within a defined deadline $w$. 
In many cases, an exact expression for the delay violation probability is complicated to derive. 
However, queueing analysis can give statistical bounds on this function. 
In particular, the stochastic network calculus framework contains tools that are appropriate for deriving an upper bound on $p_i(w)$. 
Such delay bounds are particularly suitable for performance evaluation in mission-critical networks since they provide upper limits on the delay violation probability, i.e., a real system operating under the assumed conditions will certainly achieve a better delay performance.

\paragraph{Stochastic Network Calculus} % (fold)
\label{par:stochastic_network_calculus}

Stochastic network calculus (SNC) is a mathematical framework that allows us to analyze input-output relationships of stochastic queueing systems through, for example, performance bounds on delay or backlog given arrival and service distributions. 
For a complete overview of stochastic network calculus, we refer to \cite{Fidler2015}. 
The work in~\cite{Zubaidy2016} developed the stochastic network calculus framework for wireless fading links by observing that the analysis is simplified by converting the bivariate stochastic processes $A(\tau,t)$, $S(\tau,t)$ and $D(\tau,t)$ into $\mathcal{A}(\tau,t)\triangleq e^{A(\tau,t)}$, $\mathcal{S}(\tau,t)\triangleq e^{S(\tau,t)}$ and $\mathcal{D}(\tau,t)\triangleq e^{D(\tau,t)}$. 
This transformation allows the characterization of the random service process in terms of the varying instantaneous SNR due to fading. 
This is referred to as transforming the bit-domain processes into the SNR-domain since the processes become linear in the instantaneous SNR $\gamma_k$ instead of logarithmic. 
Arrival processes in the SNR-domain can then be seen as instantaneous SNR demands. 
The performance bounds, which can be seen as variations of moment bounds, are derived in terms of Mellin transforms of the involved queueing processes.
The Mellin transform of a random variable $X$, closely related to the moment-generating function (MGF), is defined as $\mathcal{M}_{X}(s) = \mathbb{E}[X^{s-1}]$.

\paragraph{SNC Delay Bound}
\label{par:snc_delay_bound}



The upper bound on the delay violation probability we utilize in this paper is given by the following lemma:
\begin{lemma}
\label{lem:kernel}
For $s>0$ and under the stability condition $\MelA(1+s)\MelS(1-s)<1$,

\begin{equation}
	p(w) \leq \min_{s}\frac{\MelS(1-s)^w}{1-\MelA(1+s)\MelS(1-s)}
	\label{eq:snc_delay_bound}
\end{equation}
%
where $\MelS(s) \triangleq \E[e^{s_k(s-1)}]$ and $\MelA(s) \triangleq \E[e^{a_k(s-1)}]$ are the Mellin transforms of the independent SNR-domain service and arrival processes, respectively.
\end{lemma}
\begin{proof}
See~\cite[Theorem 1]{Zubaidy2016}.
\end{proof}
%
The upper bound \eqref{eq:snc_delay_bound} can be shown to be a convex function for every $s$ in the stability interval $\MelA(1+s)\MelS(1-s)<1$~\cite[Theorem 1]{Zubaidy2016_convex}. 
However, no analytical tools from convex optimization can be applied, and therefore, one typically resorts to a numerical grid search.

\subsection{Queueing Model for Distributed System}

In this work, we will assume constant arrivals of $\gamma$ bits per frame.
Hence, the arrival process is deterministic and the Mellin transform of the SNR-domain arrival process can easily be found to be $\MelA(s) = e^{\gamma(s-1)}$. 

We divide the flow of DTA transmissions from the devices to the CPU into a three-step process:

\begin{enumerate}
\item Given that device $i$ is scheduled $N_k$, given by \eqref{eq:N_k}, PHY-layer resources, we assume that it encodes and transmits $RN_k$ bits from the buffer where $R$ is a fixed rate.

\item The distributed arrays receive the transmission and either (i) forward the samples to the CPU for \textit{central processing} or (ii) decode transmissions independently using \textit{local processing} and forward the data to the CPU. See also Section~\ref{par:phy_layer_processing}.

\item The CPU carries out the authentication hypothesis test based on the CSI. If the CPU decides $\Hyp_1$ the DTA message is accepted and passed to higher layers. 
If, on the other hand, the CPU decides $\Hyp_0$, the DTA message is rejected and, thus, cannot be considered successfully received at Bob.
\end{enumerate}

To model the service process consisting of steps 1-3 above, we use the following definition of the instantanous service

\begin{equation}
s_k = \begin{cases}
R N_k & \text{if} \quad X_{k,i} = 1 \\
0 & \text{if} \quad X_{k,i} = 0
\end{cases},
\label{eq:general_service_model}
\end{equation}
%
where $X_{k,i}$ is a stochastic indicator of successful reception at the CPU.
This model \eqref{eq:general_service_model} gives us two simple interfaces, $N_k$ and $X_{k,i}$, whose distributions will determine the performance of the link.
In the rest of this section we will denote the distribution of $X_{k,i}$ using $p_X=\prob(X_{k,i}=0) = 1-\prob(X_{k,i}=1)$.
Recall that the service process Mellin transform $\MelS(s) \triangleq \E[e^{s_k(s-1)}]$, which together with \eqref{eq:general_service_model} gives us

\begin{equation}
	\MelS(s) = e^{RN_k(s-1)}(1-p_X) + p_X
	\label{eq:service_mellin}
\end{equation}

\paragraph{MAC-Layer Attack Impacts} % (fold)
\label{par:attacker_impacts}
The result \eqref{eq:service_mellin} is conditioned on the number of scheduled resources $N_k$ that in general is a stochastic variable.
For instance, if the attacker launch a Sybil attack (as discussed in Section~\ref{sub:adversarial_strategies}), the scheduled resources will depend on the success probability of the launched attack.
We have previously derived the resulting Mellin-transform under the attack strategies \textit{dissasociation attack}~\cite[Corollary 1]{Forssell2019} and \textit{Sybil attack}~\cite[Corollary 2]{Forssell2019}.
Effectively, the Mellin transform \eqref{eq:service_mellin} correspond to the \textit{baseline} Mellin transform in \cite[Corrolary 1]{Forssell2019} and extension to the discussed MAC-layer attack strategies follows equivalently.


\subsection{Service Outage Model 1: Centralized Decoding} % (fold)
\label{sec:outage_1}

With access to digital sample-streams from the distributed arrays, the CPU is able to extract the channel observations $\mathbf{y}_{1,k}(n),\cdots,\mathbf{y}_{\Na,k}(n)$ and channel states $\tilde{\h}_{1,k},\cdots,\tilde{\h}_{\Na,k}$ from each antenna array.
In the centralized processing scheme, we assume that the CPU uses maximum-ratio-combining (MRC) with the observations from all the arrays.
This yields an effective signal-to-noise ratio (SNR) $\gamma(\tilde{\h}_k) = \frac{\|\tilde{\h}_k\|^2}{\Na N_0}$ with $\tilde{\h}_k =[\tilde{\h}_{1,k}^T,\cdots,\tilde{\h}_{\Na,k}^T]^T $.
Assuming the devices encode their transmissions with rate $R$, the CPU can successfully decode the transmission given that $R<C_k$ where we in this paper adopt the Shannon capacity $C_k = \log(1+\gamma_k)$.
Let $\mathcal{D}(\tilde{\h}_k)$ denote the centralized authentication discriminant function.
The probability of non-zero service is

\begin{equation}
\begin{aligned}
\prob(X_k=1) = \prob(\mathcal{D}(\tilde{\h}_k)<T,\gamma_k(\tilde{\h}_k) > 2^R-1) \\
\end{aligned}
\label{eq:X_k}
\end{equation}
%
i.e., the probability that the packet is authenticated successfully and that the instantaneous SNR is above the rate-dependent threshold.
Based on~\eqref{eq:X_k}, we provide an upper bound on the outage probability in the following lemma:
\begin{lemma}[Outage probability bound]
	The probability of service outage can in the centralized decoding model be upper bounded by
	\begin{equation}
		p_X \leq \pFA(T)+p_{\text{out}}(R)
	\end{equation}
	where $p_{\text{out}} = \prob(\gamma_k(\tilde{\h}_k) < 2^R-1)$ is the SNR outage probability.
\end{lemma}
%
Furthermore, we provide an exact result which holds under certain rate-threshold relationships

%---------------------------------------->
\begin{lemma}
%---------------------------------------->
Under the assumption

\begin{equation}
	\sqrt{2^R-1}<\sqrt{\frac{T}{2\lambda_{\min}(\Cov^{-1})}}-\|\mean\|,
	\label{eq:rate_threshold}
\end{equation}
%
the outage probability in the centralized decoding case is $p_X = \pFA(T)$.
\end{lemma}
%---------------------------------------->
\begin{proof}
Given that $\mathcal{D}(\tilde{\h})<T$, it follows that

\begin{equation}
	\begin{aligned}
		T>\mathcal{D}(\tilde{\h}) = 2(\tilde{\h}-\mean)^\dag\Cov^{-1}(\tilde{\h}-\mean)\\
		\geq 2\lambda_{\min}(\Cov^{-1})\|\tilde{\h}-\mean\|^2 \geq 
		2\lambda_{\min}(\Cov^{-1})| \|\tilde{\h}\| -\|\mean\| |^2
	\end{aligned}
	\label{eq:norm_bound}
\end{equation}
%
where we have used the triangle inequality and $\lambda_{\min}(\Cov^{-1})$ represents the minimum eigenvalue of $\Cov^{-1}$.
Hence, we can by rearranging \eqref{eq:norm_bound} get that for every $\tilde{\h}\in\mathcal{C}^{\Na\NRx}$ such that $\mathcal{D}(\tilde{\h})<T$, we have 

\begin{equation}
	\|\tilde{\h}\|^2 < \left(\sqrt{\frac{T}{2\lambda_{\min}(\Cov^{-1})}}-\|\mean\|\right)^2
\end{equation}
%
Then we note that if \eqref{eq:rate_threshold} holds, then $\prob(\gamma_k(\tilde{\h}_k) > 2^R-1|\mathcal{D}(\tilde{\h}_k)<T)=1$ and

\begin{equation}
\begin{aligned}
\prob(X_k=1) = \prob(\gamma_k(\tilde{\h}_k) > 2^R-1|\mathcal{D}(\tilde{\h}_k)<T)\prob(\mathcal{D}(\tilde{\h}_k)<T)  \\
= \prob(\mathcal{D}(\tilde{\h}_k)<T) = 1-\pFA(T).
\end{aligned}
\end{equation}
%---------------------------------------->
\end{proof}
%---------------------------------------->

\subsection{Service Outage Model 2: Local Decoding} 
\label{sec:outage_2}
If, on the other hand, PHY-layer processing is distributed to local processing at the antenna arrays, we assume that the arrays independently perform MRC using the locally received symbols.
Specifically, array $j$ uses $\y_k^{(j)}(n)$ for MRC with the local SNR $\gamma_{k}^{(j)} = \frac{\|\h_k^{(j)}\|^2}{N_0}$.
Similar to the centralized case, we assume that the array can successfully decode the transmission given that $R<C_k^{(j)}$, with $C_k^{(j)} = \log(1+\gamma_{k}^{(j)})$.
Given succesfull decoding, the array forward the data to the CPU over an error-free channel.
Hence, we can assume that the CPU successfully decodes the transmission if \textit{any} array is able to decode it.
This allows us to formulate an upper bound on the service outage probability in the following lemma:

\begin{lemma}
	The probability of service outage ($X_{k,i}=0$) can in the local decoding model be upper bounded by
	\begin{equation}
		p_X \leq \pFA(T)+\prod_{j=1}^{\Ka}p_{\text{out}}^{(j)}(R)
	\end{equation}
	where $p_{\text{out}}^{(j)}(R) = \prob(\gamma_k^{(j)} < 2^R-1)$ is the per-array SNR outage probability.
	
\end{lemma}

